Self-Alignment for Factuality: Mitigating Hallucinations in LLMs via Self-Evaluation

Despite showing increasingly human-like abilities, large language models (LLMs) often struggle with factual inaccuracies, i.e. "hallucinations", even when they hold relevant knowledge. To address these hallucinations, current approaches typically necessitate high-quality human factuality annotations. In this work, we explore Self-Alignment for Factuality, where we leverage the self-evaluation capability of an LLM to provide training signals that steer the model towards factuality. Specifically, we incorporate Self-Eval, a self-evaluation component, to prompt an LLM to validate the factuality of its own generated responses solely based on its internal knowledge. Additionally, we design Self-Knowledge Tuning (SK-Tuning) to augment the LLM's self-evaluation ability by improving the model's confidence estimation and calibration. We then utilize these self-annotated responses to fine-tune the model via Direct Preference Optimization algorithm. We show that the proposed self-alignment approach substantially enhances factual accuracy over Llama family models across three key knowledge-intensive tasks on TruthfulQA and BioGEN.

==> floats/tables/table_cluster_selection.tex <==
\begin{table}[th]
\setlength\tabcolsep{1.5pt}
  \centering
  \begin{threeparttable}
  \fontsize{8}{9}
  \selectfont
    \begin{tabular}{lccccccccc}
    \toprule
    \multirow{2}{*}{Model}& \multirow{2}{*}{\makecell[c]{Selection of \\ Preferred Res.}}&
    \multicolumn{3}{c}{\texttt{TruthfulQA}}
    \cr\cmidrule(lr){3-5}
     &&\% $\mathtt{True}$ &\% $\mathtt{Info}$&\% $\mathtt{True^{*}Info}$\cr
    \midrule
    % 0.3876712329, 0.9575342466, 0.3506849315
    \textsc{LLAMA-7B} &- &30.40 & \textbf{96.30}& 26.90 \\
    %  + \iti{} \cite{li2023inferencetime} &\Checkmark &25.90 &49.10 &-&43.50&- &-\\
    % + \dola{} \cite{chuang2023dola} &\Checkmark &32.20&42.10&98.30&40.80&62.00&62.20\\
    % + \textsc{SC} \cite{tian2023finetuning, wang2023selfconsistency} \\
    + \ski{} &S-Max-P(True) &40.82 & 95.34& 36.58\\
    + \ski{} &Ave-P(True) &\textbf{47.81} & 90.27& 38.90\\
    + \ski{} (Ours) &Max-P(True) &47.12 & 96.03 & \textbf{43.97}\\
    % \midrule
    % \textsc{LLAMA2-7B}  & & 51.78 & 90.00&42.05\\
    % % + \lmmk{} \cite{kadavath2022language} &&32.74 &-\\
    % + \textsc{SC} \cite{tian2023finetuning, wang2023selfconsistency}** &&39.45& 97.53& 36.99 \\
    % + \ski{} (Ours)** & &44.93& 97.12& 43.01\\

    \bottomrule  
    \end{tabular}
  \end{threeparttable}
  \caption{Evaluation results on exploring the variations in the selection of the preferred responses (res.).}
  \label{tab:ablation_tab}
  \vspace{-1mm}
\end{table}

==> floats/tables/table_clustering_vs_ranking.tex <==
\begin{table}[th]
\setlength\tabcolsep{1.5pt}
  \centering
  \begin{threeparttable}
  \fontsize{8}{9}
  \selectfont
    \begin{tabular}{lccccccccc}
    \toprule
    \multirow{2}{*}{Model}& \multirow{2}{*}{\makecell[c]{Selection of \\ Pre./Dispre. Res.}}&
    \multicolumn{3}{c}{\texttt{TruthfulQA}}
    \cr\cmidrule(lr){3-5}
     &&\% $\mathtt{True}$ &\% $\mathtt{Info}$&\% $\mathtt{True^{*}Info}$\cr
    \midrule
    % 0.3876712329, 0.9575342466, 0.3506849315
    \textsc{LLAMA2-7B} &- &\textbf{50.41} & 88.22 & 39.04 \\
    + \ski{} &Sem.-Clustering &48.49& \textbf{98.77}& 47.53\\
    + \ski{} (Ours) &Purely-Ranking &55.07& \textbf{98.08}& \textbf{53.42}\\
    % \midrule
    % \textsc{LLAMA2-7B}  & & 51.78 & 90.00&42.05\\
    % % + \lmmk{} \cite{kadavath2022language} &&32.74 &-\\
    % + \textsc{SC} \cite{tian2023finetuning, wang2023selfconsistency}** &&39.45& 97.53& 36.99 \\
    % + \ski{} (Ours)** & &44.93& 97.12& 43.01\\

    \bottomrule  
    \end{tabular}
  \end{threeparttable}
  \caption{Evaluation results on exploring the variations in the selection of the preferred/dispreferred responses (res.).}
  \label{tab:ablation_tab}
  \vspace{-1mm}
\end{table}

==> floats/tables/table_main_v0213.tex <==

% \begin{table*}[!t]
% \setlength\tabcolsep{1.5pt}
%   \centering
%   \begin{threeparttable}
%   \fontsize{8}{8}
%   \selectfont
%     \begin{tabular}{lccccccccc}
%     \toprule
%     \multirow{2}{*}{Model}& \multirow{2}{*}{\makecell[c]{Labeled \\ In-dom. data}}&
%     \multicolumn{4}{c}{\texttt{TruthfulQA}}
%      &\multicolumn{4}{c}{\texttt{BioGEN}}\cr\cmidrule(lr){3-6} \cmidrule(lr){7-10}
%       &&\% $\mathtt{MC}$ $\mathtt{acc.}$&\% $\mathtt{True}$ &\% $\mathtt{Info}$&\% $\mathtt{True^{*}Info}$&\# $\mathtt{Cor.}$&\# $\mathtt{Incor.}$ &\% $\mathtt{Res.}$&\% $\mathtt{FActScore}$\cr
%     \midrule
%     % 0.3876712329, 0.9575342466, 0.3506849315
%     \textsc{LLAMA-7B$^{*}$}  &-& 25.60 &30.40 & 96.30& 26.90 &7.70&16.92&98.00&30.72\\
%     + \textsc{SFT$^{*}$} &\Checkmark  & 24.20 & 47.10 & - & 36.10 &8.52&16.52&98.00&32.17 \\
%      + \iti{}$^{*}$ \cite{li2023inferencetime} &\Checkmark &25.90 &\textbf{49.10} &-&43.50&- &-&-&-\\
%     + \dola{}$^{*}$ \cite{chuang2023dola} & \Checkmark &32.20&42.10&\textbf{98.30}&40.80&7.46&13.70&99.00&33.91\\
%     + \textsc{FactTune-MC} \cite{tian2023finetuning} &&-&-&-&-&\textbf{10.98}&21.33&99.00&30.92\\
%     + \ski{} (Ours) &&\textbf{45.48} &47.40 & 97.26 & \textbf{45.75}&8.54&\textbf{13.49}&\textbf{100.00}&\textbf{38.28}\\
%     % + \ski{} (+bigbench) &&- &46.30 & 97.12 & 44.11\\
%     % + \ski{w.golden\_labels} (Ours) &\Checkmark&&0.5794520547945206& 0.8383561643835616& 0.42054794520547945\\
%     \midrule

%     \textsc{LLAMA2-7B}  &-& 28.90 & \textbf{50.41} & 88.22 & 39.04&8.84&12.65&99.00&40.54\\
%     + \dola{} \cite{chuang2023dola} &\Checkmark &31.10&47.53 & 94.66 & 42.60&8.74&11.85&72.00&38.99 \\
%     + \textsc{FactTune-MC} \cite{tian2023finetuning} &&-&-&-&-&\textbf{12.64}&16.16&100.00&42.71 \\
%     + \textsc{Finetune-Naive-P(True)} &&43.15 & 44.52 & 94.93 & 41.10 & 8.46 & 11.17 & \textbf{100.00} & 42.73 \\
%     + \ski{} (Ours) &&\textbf{44.10} &55.07& \textbf{98.08}& \textbf{53.42}&12.12&\textbf{14.44}&99.00&\textbf{46.50}\\
%     % \midrule
%     % \textsc{LLAMA2-7B-CHAT}  &-& 33.56&63.42&91.64&55.34&10.41&15.42 &83.00& 39.59\\
%     % 48.49& \textbf{98.77}& \textbf{47.53} 8.68&\textbf{9.83}&\textbf{100.00}&\textbf{46.01}
%     \bottomrule  
%     \end{tabular}
%   \end{threeparttable}
%   \caption{Evaluation results on three tasks: multi-choice QA (employing 6-shot prompting for baseline methods and 5-shot prompting for \ski{}) on TruthfulQA, short-form open-ended generation (using 6-shot prompting) on TruthfulQA, and long-form open-ended generation (utilizing 5-shot prompting) on BioGEN. For the multi-choice QA and short-form open-ended generation tasks, results marked with an asterisk are cited from \citet{li2023inferencetime, chuang2023dola}. The remaining results of the baseline methods are reproduced following the approaches described in \citet{chuang2023dola, tian2023finetuning}.}
%   \label{tab:main_tab}
%   \vspace{-1mm}
% \end{table*}



\begin{table*}[!t]
	\setlength\tabcolsep{1.5pt}
	\centering
	\begin{threeparttable}
		\fontsize{8}{8.5}
		\selectfont
		\begin{tabular}{lccccccccc}
			\toprule
			\multirow{2}{*}{Model}& \multirow{2}{*}{\makecell[c]{Labeled \\Task-Specific\\ Data}}&
			\texttt{TruthfulQA (MC)} & \multicolumn{3}{c}{\texttt{TruthfulQA (Gen.)}}
			&\multicolumn{4}{c}{\texttt{BioGEN (Long-Form Gen.)}}\cr\cmidrule(lr){3-3} \cmidrule(lr){4-6} \cmidrule(lr){7-8}
			                                                 &            & \%  $\mathtt{Accuracy}$ & \% $\mathtt{True}$ & \% $\mathtt{Info}$ & \% $\mathtt{True^{*}Info}$ & \% $\mathtt{Res.}$ & \% $\mathtt{FActScore}$\cr 
			\midrule
			% 0.3876712329, 0.9575342466, 0.3506849315
			\textsc{\llama{}$^{*}$}                          & -          & 25.60                            & 30.40              & 96.30              & 26.90                                    & 98.00              & 30.72                      \\
			+ \textsc{SFT$^{*}$}                             & \Checkmark & 24.20                            & 47.10              & -                  & 36.10                                & 98.00              & 32.17                      \\
			+ \iti{}$^{*}$ \cite{li2023inferencetime}        & \Checkmark & 25.90                            & \textbf{49.10}     & -                  & 43.50                                      & -                  & -                          \\
			+ \dola{}$^{*}$ \cite{chuang2023dola}            &\Checkmark & 32.20                            & 42.10              & \textbf{98.30}     & 40.80                              & 99.00              & 33.91                      \\
			+ \textsc{FactTune-MC} \cite{tian2023finetuning} &            & -                                & -                  & -                  & -                                  & 99.00              & 30.92                      \\
   \hdashline
   \noalign{\vskip 0.07cm} % Adds a small vertical space
   % \multicolumn{10}{l}{\cellcolor{lightgray!25}{+ \ski{}}}\cr 
   \multicolumn{10}{l}{\textcolor{lightgray!99}{\textit{Self-Alignment for Factuality (Ours)}}}\cr 
			w/ \selfskt{}                                &            & \textbf{45.48}                   & 47.40              & 97.26              & \textbf{45.75}           & \textbf{100.00}    & \textbf{38.28}             \\
			% + \ski{} (+bigbench) &&- &46.30 & 97.12 & 44.11\\
			% + \ski{w.golden\_labels} (Ours) &\Checkmark&&0.5794520547945206& 0.8383561643835616& 0.42054794520547945\\
			\midrule
			
			\llamaa{}                               & -          & 28.90                            & 50.41    & 88.22              & 39.04                      & 8.84               & 12.65                & 99.00              & 40.54                      \\
			+ \dola{} \cite{chuang2023dola}                 &\Checkmark & 31.10                            & 47.53              & 94.66              & 42.60                      & 8.74               & 11.85                & 72.00              & 38.99                      \\
			+ \textsc{FactTune-MC} \cite{tian2023finetuning} &            & -                                & -                  & -                  & -                          & \textbf{12.64}     & 16.16                & 100.00             & 42.71                      \\
   \hdashline
   \noalign{\vskip 0.07cm} % Adds a small vertical space
   \multicolumn{10}{l}{\textcolor{lightgray!99}{\textit{Self-Alignment for Factuality (Ours)}}}\cr 
        % \multicolumn{10}{l}{\cellcolor{lightgray!25}{+ \ski{}}}\cr  
		w/ \selfpt{}             &            & 43.15                            & 44.52              & 94.93              & 41.10                      & 8.46               & \textbf{11.17}                & \textbf{100.00}    & 42.73                      \\
		w/ \selfskt{}                           &            & \textbf{44.10}                   & \textbf{55.07}              & \textbf{98.08}     & \textbf{53.42}             & 12.12              & 14.44       & 99.00              & \textbf{46.50}           \\
			% \midrule
			% \textsc{LLAMA2-7B-CHAT}  &-& 33.56&63.42&91.64&55.34&10.41&15.42 &83.00& 39.59\\
			% 48.49& \textbf{98.77}& \textbf{47.53} 8.68&\textbf{9.83}&\textbf{100.00}&\textbf{46.01}
			\bottomrule  
		\end{tabular}
	\end{threeparttable}
	% \caption{Few-shot evaluation results on three distinct tasks: 6-shot prompting results of the MCQA and short-form generation tasks on \texttt{TruthfulQA}, and 5-shot prompting results of the long-form generation task on \texttt{BioGEN}.\footnotemark Results on \texttt{TruthfulQA} marked with an asterisk are cited from~\protect\citet{li2023inferencetime, chuang2023dola}. The remaining results of \dola{} and \textsc{FactTune-MC} are reproduced following~\protect\citet{chuang2023dola, tian2023finetuning}.}
\caption{Few-shot evaluation results on three distinct tasks: 6-shot prompting results of the MCQA and short-form generation tasks on \texttt{TruthfulQA}, and 5-shot prompting results of the long-form generation task on \texttt{BioGEN}.\protect\footnotemark Results on \texttt{TruthfulQA} marked with an asterisk are cited from~\protect\citet{li2023inferencetime} and~\protect\citet{chuang2023dola}. The remaining results of \dola{} and \textsc{FactTune-MC} are reproduced following~\protect\citet{chuang2023dola} and~\protect\citet{tian2023finetuning}.}
	\label{tab:main_tab}
	\vspace{-1mm}
\end{table*}

\footnotetext{We use the default QA prompt as in~\protect\citet{lin-etal-2022-truthfulqa, li2023inferencetime, chuang2023dola} on \texttt{TruthfulQA} and the prompt generated by GPT-4~\protect\cite{openai2023gpt4} on \texttt{BioGEN} (Table \ref{tab:biogen_prompt} in Appendix \ref{sec:imple_details}).}


==> floats/tables/table_pairwise_vs_top50.tex <==
\begin{table}[th]
\setlength\tabcolsep{1.5pt}
  \centering
  \begin{threeparttable}
  \fontsize{8}{9}
  \selectfont
    \begin{tabular}{lccccccccc}
    \toprule
    \multirow{2}{*}{Model}& \multirow{2}{*}{\makecell[c]{Training Strategy \\ with DPO}}&
    \multicolumn{4}{c}{\texttt{BioGEN}}
    \cr\cmidrule(lr){3-6}
     &&\# $\mathtt{Cor.}$&\# $\mathtt{Incor.}$ &\% $\mathtt{Res.}$&\% $\mathtt{FActScore}$\cr
    \midrule
    % 0.3876712329, 0.9575342466, 0.3506849315
    \textsc{LLAMA2-7B} &- & 8.84&12.65&99.00&40.54\\
    + \ski{} &Pairwise &11.03 & 14.26 & 97.00& 43.41\\
    + \ski{} (Ours) &Top-50\%& 12.12&\textbf{14.44}&99.00&\textbf{46.50} \\
    % 8.68&\textbf{9.83}&\textbf{100.00}&\textbf{46.01}\\


    \bottomrule  
    \end{tabular}
  \end{threeparttable}
  \caption{Evaluation results on exploring the variations in the selection of the preferred/dispreferred responses (res.).}
  \label{tab:ablation_tab}
  \vspace{-1mm}
\end{table}
